When SRv6 meets 5G Core: Implementation and Deployment of a Network Service Chaining Function in SmartNICs

Currently, we have witnessed a myriad of solutions that benefit from programmable hardware. The 5G Core (5GC) can and should also benefit from such paradigm to offload certain functions to the dataplane. In this work, we designed and implemented a P4-based solution for traffic identification and chaining using the Netronome Agilo SmartNIC. The solution here presented is deployed in-between the RAN and UPF (User Plane Function) so that traffic coming from the RAN is identified and chained using SRv6 based on different rules defined by the control plane. The traffic identification and the construction of the SRv6 list of segments are done entirely in the SmartNIC. A minimalist Proof-of-Concept (PoC) was deployed and evaluated to show that this function is perfectly capable to build service function chainings in a transparent and efficient way.

==> 4Conclusion.tex <==
\section{Conclusion}
\label{cap-conclusion}

In our initial tests, we can conjecture that the INCA perform the task of classifying the packages perfectly, constructing and removing the SRv6 header and also the correct routing between functions. We were able to create two different paths with three functions, where each path passes through only two of these.

In the next works we will to make more tests with more functions and chainings, we want to build chainings with more than two functions, in addition to collecting performance data.

==> Background.tex <==
\section{Background}
\label{cap-backgroud}

\subsection{5G core and infrastructure}

To satisfy new consumer, service and business demands, the infrastructure of 5G impose a wider range of requirements than existing services do nowadays \cite{Ordonez-Lucena2017}. To achieve this, the 5G new core was built with control and user plane separation, service-based architecture, network slicing and it is design to be cloud native. 


In Figure 1 we can see 5G components. All of these components are now softwarized. This brings more flexibility to the architecture. 

\begin{figure}[h]
    \centering
    \includegraphics[width=8cm]{images/5gc.png}
    \caption{5G INFRASTRUCTURE}
    \label{fig:5ginfra}
\end{figure}

One of the most important concept is the PDU Session concept, that is, a logical network between a UE and a Data Network (reachable via a UPF) that provides a PDU connectivity service. 

\subsection{SEGMENT ROUTING OVER IPV6 (SRV6)}

SRV6 is the IPv6 data-plane instantiation of Segment Routing \cite{rfc8402}. works like a extension of IPv6 header, that is created with a segment list (ipv6 address) and a pointer to identify which segment is active. Every time that the packet pass through a segment endpoint (SR-capable nodes whose address is in the IPv6 destination address) the pointer decrease, and the new segment-id of the segment list is copy to the destination address. If the packet pass through a non srv6-aware device, the forwarding is done normally with the destination address. This way, SRV6 integrates both the application and the underlying transport layer into a single protocol, allowing operators to optimize the network in a simplified manner and removing forwarding state from the network.\cite{ietf-dmm-srv6-mobile-uplane-07} 

\begin{figure}[ht]
    \centering
    \includegraphics[width=6cm]{images/ipv6_srv6_header.png}
    \caption{IPv6 + SRv6 Header}
    \label{fig:header}
\end{figure}
